MCBeth: A Measurement Based Quantum Programming Language

Gate-based quantum programming languages are ubiquitous but measurement-based languages currently exist only on paper. This work introduces MCBeth, a quantum programming language which allows programmers to directly represent, program, and simulate measurement-based and cluster state computation by building upon the measurement calculus. While MCBeth programs are meant to be executed directly on hardware, to take advantage of current machines we also provide a compiler to gate-based instructions. We argue that there are clear advantages to measurement-based quantum computation compared to gate-based when it comes to implementing common quantum algorithms and distributed quantum computation.

==> Makefile <==
PAPER = main
VERBOSE = 0

# directories
FIGURE_DIR = figures
OUTPUT_DIR = output
STYLE_DIR = style
TEXT_DIR = text
BIB_OUT_FILE = $(OUTPUT_DIR)/bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR)/sty:$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode 
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true 

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat $(OUTPUT_DIR)/*.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)
PRINT_BIBTEX_NOTE = if [ -s $(BIB_OUT_FILE) ]; then \
                    echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."; fi

#formats
NORM=
BOLD=
PS2PDF_LABEL   =[ps2pdf   ] 
DVIPS_LABEL    =[dvips    ] 
LATEX_LABEL    =[latex    ] 
BIBTEX_LABEL   =[bibtex   ] 
NOTE_LABEL     =[note     ] 
MAKEINDEX_LABEL=[makeindex] 
RM_LABEL       =[rm       ] 

SHELL:=/bin/bash

all: $(OUTPUT_DIR)/$(PAPER).pdf

show: $(OUTPUT_DIR)/$(PAPER).pdf
	@evince $(OUTPUT_DIR)/$(PAPER).pdf &

$(OUTPUT_DIR)/$(PAPER).pdf: $(TEXT_DIR)/$(PAPER).tex                      \
                            $(shell find $(TEXT_DIR) -regex "[^.]*.tex")  \
                            $(shell find $(TEXT_DIR) -regex  "[^.]*.bib") \
                            $(shell find $(STYLE_DIR) -regex "[^.]*.tex") \
                            $(shell find $(FIGURE_DIR) -name "*.pdf") 
	@mkdir -p $(OUTPUT_DIR)

	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS) output/$(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi 
	@-$(PRINT_BIBTEX_WARNINGS)
	@-$(PRINT_BIBTEX_NOTE)

#	@echo "$(MAKEINDEX_LABEL)Building index..."
#	@makeindex $(MAKEINDEX_OPTS) $(OUTPUT_DIR)/$(PAPER).idx || \
#		(rm -f $@ && exit 1)

	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

#	@echo "$(LATEX_LABEL)Performing ternary latex..."
#	@TEXINPUTS=$(TEX_PATH) \
#		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
#			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)

clean:
	@echo '$(RM_LABEL)Cleaning project...'
	@rm -fr $(OUTPUT_DIR)


==> blocks.tex <==
%% H makes sure that it's at the end of the document


\begin{figure}[H]
  \scalebox{0.9}{
  \begin{minipage}{0.99\textwidth}
    
  \begin{flushleft}
    Cluster 1: ``Linear-3''
  \end{flushleft}
  
  
  \begin{minipage}{0.48\textwidth}
    \centering
    \begin{tikzpicture}  
      [scale=.9,auto=left,every node/.style={circle,fill=blue!20}]
        
      \node (a1) at (1,1) {$q_1$};  
      \node (a2) at (3,1) {$q_2$};  
      \node (a3) at (5,1) {$q_3$};
      
      \draw (a1) -- (a2); 
      \draw (a2) -- (a3);

    \end{tikzpicture}
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
    {
      % definitions for the circuit elements

      \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
      \def\gBxA{\op{R_x(-\beta)}\w\A{gBxA}}

      % definitions for bit labels and initial states

      \def\bA{\qv{q_{3}}{q_1}}

      % The quantum circuit as an xymatrix

      \xymatrix@R=5pt@C=10pt{
          \bA & \gAxA &\gBxA &\n
      %
      % Vertical lines and other post-xymatrix latex
      %
      }
    }
  \end{minipage}
  \begin{flushright}
    $J(\alpha)(q_1, q_2); J(\beta)(q_2,q_3)$
  \end{flushright}
  \vspace{0mm}

  \begin{flushleft}
    Cluster 2: ``Linear-4''
  \end{flushleft}
  \begin{minipage}{0.40\textwidth}
    \centering
    \centering
    \begin{tikzpicture}  
      [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
        
      \node (a1) at (1,1) {$q_1$};  
      \node (a2) at (2.5,1) {$q_2$};  
      \node (a3) at (4,1) {$q_3$};
      \node (a4) at (5.5,1) {$q_4$};
      
      \draw (a1) -- (a2); 
      \draw (a2) -- (a3);
      \draw (a3) -- (a4);

    \end{tikzpicture}  
  \end{minipage}\hfill
  \begin{minipage}{0.40\textwidth}
    {
      \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
      \def\gBxA{\op{R_x(-\beta)}\w\A{gBxA}}
      \def\gCxA{\op{R_z(-\gamma)}\w\A{gCxA}}
      \def\gDxA{\op{H}\w\A{gDxA}}

      % definitions for bit labels and initial states

      \def\bA{\qv{q_{4}}{q_1}}

      % The quantum circuit as an xymatrix

      \xymatrix@R=5pt@C=10pt{
          \bA & \gAxA &\gBxA &\gCxA &\gDxA &\n
      %
      % Vertical lines and other post-xymatrix latex
      %
      }
    }
  \end{minipage}
  \begin{flushright}
    $J(\alpha)(q_1, q_2); J(\beta)(q_2,q_3); J(\gamma)(q_3,q_4)$
  \end{flushright}
  \vspace{0mm}

  \begin{flushleft}
    Cluster 3: ``Horseshoe''
  \end{flushleft}
  \begin{minipage}{0.48\textwidth}
    \centering
    \begin{tikzpicture}  
      [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
        
      \node (a1) at (1,3) {$q_1$};
      \node (a2) at (1,1) {$q_2$};  

      \node (a3) at (3,3) {$q_3$};
      \node (a4) at (3,1) {$q_4$};  
      
      \draw (a1) -- (a2); 
      \draw (a1) -- (a3);
      \draw (a2) -- (a4);

    \end{tikzpicture} 
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
    {
      \def\gAxA{\b\w\A{gAxA}}
      \def\gAxB{\b\w\A{gAxB}}
      \def\gBxA{\op{R_z(-\alpha)}\w\A{gBxA}}
      \def\gBxB{\op{R_z(-\beta)}\w\A{gBxB}}
      \def\gCxA{\op{H}\w\A{gCxA}}
      \def\gCxB{\op{H}\w\A{gCxB}}
      
      % definitions for bit labels and initial states
      
      \def\bA{\qv{q_{3}}{q_1}}
      \def\bB{\qv{q_{4}}{q_2}}
      
      % The quantum circuit as an xymatrix
      
      \xymatrix@R=5pt@C=10pt{
          \bA & \gAxA &\gBxA &\gCxA &\n
      \\  \bB & \gAxB &\gBxB &\gCxB &\n
      %
      % Vertical lines and other post-xymatrix latex
      %
      \ar@{-}"gAxA";"gAxB"
      }
    }
  \end{minipage}
  \begin{flushright}
    $CZ(q_1,q_2); J(\alpha)(q_1, q_3); J(\beta)(q_2,q_4)$
  \end{flushright}
  \vspace{0mm}

  \begin{flushleft}
    Cluster 4: ``Reverse Horseshoe''
  \end{flushleft}
  \begin{minipage}{0.48\textwidth}
    \centering
    \begin{tikzpicture}  
      [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
        
      \node (a1) at (1,3) {$q_1$};
      \node (a2) at (1,1) {$q_2$};  

      \node (a3) at (3,3) {$q_3$};
      \node (a4) at (3,1) {$q_4$};  
      
      \draw (a3) -- (a4); 
      \draw (a1) -- (a3);
      \draw (a2) -- (a4);

    \end{tikzpicture} 
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
    {
      \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
      \def\gAxB{\op{R_z(-\beta)}\w\A{gAxB}}
      \def\gBxA{\op{H}\w\A{gBxA}}
      \def\gBxB{\op{H}\w\A{gBxB}}
      \def\gCxA{\b\w\A{gCxA}}
      \def\gCxB{\b\w\A{gCxB}}
      
      % definitions for bit labels and initial states
      
      \def\bA{\qv{q_{3}}{q_1}}
      \def\bB{\qv{q_{4}}{q_2}}
      
      % The quantum circuit as an xymatrix
      
      \xymatrix@R=5pt@C=10pt{
          \bA & \gAxA &\gBxA &\gCxA &\n
      \\  \bB & \gAxB &\gBxB &\gCxB &\n
      %
      % Vertical lines and other post-xymatrix latex
      %
      \ar@{-}"gCxA";"gCxB"
      }
    }
  \end{minipage}
  \begin{flushright}
    $J(\alpha)(q_1, q_3); J(\beta)(q_2,q_4); CZ(q_1,q_2)$
  \end{flushright}
  \vspace{0mm}

  \begin{flushleft}
    Cluster 5: ``Box''
  \end{flushleft}
  \begin{minipage}{0.48\textwidth}
    \centering
    \begin{tikzpicture}  
      [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
        
      \node (a1) at (1,3) {$q_1$};
      \node (a2) at (1,1) {$q_2$};  

      \node (a3) at (3,3) {$q_3$};
      \node (a4) at (3,1) {$q_4$};  
      
      \draw (a1) -- (a2);
      \draw (a3) -- (a4); 
      \draw (a1) -- (a3);
      \draw (a2) -- (a4);

    \end{tikzpicture} 
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
    {
      \def\gAxA{\b\w\A{gAxA}}
      \def\gAxB{\b\w\A{gAxB}}
      \def\gBxA{\op{R_z(-\alpha)}\w\A{gBxA}}
      \def\gBxB{\op{R_z(-\beta)}\w\A{gBxB}}
      \def\gCxA{\op{H}\w\A{gCxA}}
      \def\gCxB{\op{H}\w\A{gCxB}}
      \def\gDxA{\b\w\A{gDxA}}
      \def\gDxB{\b\w\A{gDxB}}
      
      % definitions for bit labels and initial states
      
      \def\bA{\qv{q_{3}}{q_1}}
      \def\bB{\qv{q_{4}}{q_2}}
      
      % The quantum circuit as an xymatrix
      
      \xymatrix@R=5pt@C=10pt{
          \bA & \gAxA &\gBxA &\gCxA &\gDxA &\n
      \\  \bB & \gAxB &\gBxB &\gCxB &\gDxB &\n
      %
      % Vertical lines and other post-xymatrix latex
      %
      \ar@{-}"gAxA";"gAxB"
      \ar@{-}"gDxA";"gDxB"
      }
    }
  \end{minipage}
  \begin{flushright}
    $CZ(q_1,q_2); J(\alpha)(q_1, q_3); J(\beta)(q_2,q_4); CZ(q_1,q_2)$
  \end{flushright}
  \end{minipage}
  }
  \vspace{0mm}

  \caption{Some Basic Cluster Conversions. The cluster is shown on the left with the equivalent
  circuit shown top right and measurement calculus pattern shown bottom right. Based on work by [Walther et al., 2005]}
  %\cite{Walther_2005}
  \label{fig:clusters}
\end{figure}


==> codecomparison.tex <==


\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{MCBethStyle}{            
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\small\ttfamily,
  breakatwhitespace=false,
  breaklines=true,
  captionpos=b,
  keepspaces=true,
  numbers=none,              
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
  float=ht,
  frame=tb,
}

\subsection{MCBeth program (OCaml)}
  
  % Put it in listings, and set the font size smaller, just import a file with the python code .. move to appendix.
\lstinputlisting[language=Caml, style=MCBethStyle]{teleportation_mcbeth.ml}
  
\subsection{Qiskit Program (Gate-based)}
  
\lstinputlisting[language=python, style=MCBethStyle]{gate_based_qiskit.py}
  
\subsection{Qiskit Program (Measurement to Gate Based Translation)}
  
\lstinputlisting[language=python, style=MCBethStyle]{meas_based_qiskit.py}
  
    % # Run the circuit using Qiskit's built in simulators, 
    % # printing the results to console
    % from qiskit import IBMQ, Aer
    % sim = Aer.get_backend('aer_simulator')
    % qc.save_statevector()
    % out_vector = sim.run(qc).result().get_statevector()
    % print(out_vector)

==> old_background.tex <==

%  - Quantum computing
%  - Measurement based quantum computing
%  - PL for quantum computing
%  - Measurement calculus
\section{Background}
  \subsection{Quantum Computing}
    We now briefly review some of the basic concepts and terminology of quantum 
    computation. For a more in depth explanation, please see [TODO] or [TODO].

    \subsubsection{Dirac Notation}
      Dirac's notation, also referred to as bra-ket notation, is a common notation
      used in quantum mechanics to write quantum states. In this notation, a ``ket''
      is written as $\ket{v}$ a represents a column vector $v$. A ``bra'' is written
      as $\bra{v}$ and represents the conjugate transpose of $v$; i.e., $v^\dagger$.
      
      The inner product of two vectors $v$ and $w$ is written as $\braket{v}{w}$ in
      Dirac notation. The outer product is written as $\ket{v}\bra{w}$.
    
    \subsubsection{Quantum States}
      In contrast to classical computation's representation of information in the
      form of bits quantum computation 
      represents information in the form of quantum bits (qubits). Each qubit,
      represents a single unit of information stored in a quantum state; specifically, 
      the state is represented by a linear combination of \textit{basis states}, 
      refered to as a \textit{superposition}:
      \begin{align*}
        \ket{\psi} =  \alpha \ket{0} + \beta \ket{1} = \alpha \qstate{1}{0} 
                      + \beta \qstate{0}{1} = \qstate{\alpha}{\beta}
      \end{align*}
      where $\alpha, \beta \in \mathbb{C}$ such that $||\alpha||^2 + ||\beta||^2 = 1$.
      $\alpha$ and $\beta$ are referred to as the \textit{amplitudes} of the quantum 
      state and $\ket{0}$ and $\ket{1}$ are the \textit{basis states}.
      The $\ket{0}$ and $\ket{1}$ basis states are the most common basis states and 
      are typically referred to as the \textit{computational basis states}. In order
      for two vectors to be basis states, they must be orthogonal; i.e., for states
      $\ket{\alpha}$ and $\ket{\beta}$, $\braket{\alpha}{\beta} = 0$. 
      
      Another 
      common basis state will be important in this paper as well:
      \begin{align*}
        \ket{+} &= \frac{1}{\sqrt{2}}\ket{0} + \frac{1}{\sqrt{2}}\ket{1}\\
        \ket{-} &= \frac{1}{\sqrt{2}}\ket{0} - \frac{1}{\sqrt{2}}\ket{1}
      \end{align*}
      
      Multiple qubit states can be combined using the \textit{tensor
      product}, $\otimes$. For example, the two qubit state consisting of individual
      qubits $\ket{0}$ and $\ket{1}$ is written as $\ket{0} \otimes \ket{1}$, or in
      a shorter form as $\ket{0}\ket{1} = \ket{01}$.
    
    \subsubsection{Entanglement}
      A quantum state is \textit{entangled} when it cannot be decomposed into the 
      tensor product of each individual qubit state. For example, the state 
      \begin{align*}
        \ket{\psi} = \frac{1}{\sqrt{2}}\ket{00} + \frac{1}{\sqrt{2}}\ket{11}
      \end{align*}
      cannot be decomposed into two individual quantum states $\ket{\alpha}$ and 
      $\ket{\beta}$ such that $\ket{\psi} = \ket{\alpha} \otimes \ket{\beta}$ and is,
      therefore, considered entangled; this specific two-quantum state is referred 
      to as either an \textit{EPR pair} or \textit{Bell pair}.
    
    \subsubsection{Measurement}
      The act of measurement is a destructive operation on a quantum system
      that causes the quantum state being measured to collapse to the basis the
      measurement is performed in. For example, consider the quantum state
      $\ket{\psi} = \alpha \ket{0} + \beta \ket{1}$ and say we measure $\ket{\psi}$ 
      with respect the computational basis states, $\ket{0}$ and $\ket{1}$. If
      $\ket{\psi'}$ is the quantum state $\ket{\psi}$ post-measurement:
      \begin{align*}
        \ket{\psi'} = \begin{cases}
                        \ket{0} & \text{with probability } ||\alpha||^2\\
                        \ket{1} & \text{with probability } ||\beta||^2
                      \end{cases}
      \end{align*}
      Generally, given a state $\ket{\psi}$ and letting $\ket{\psi'}$ be the state 
      after measuring $\ket{\psi}$ with respect to the basis states $\ket{\alpha}$ 
      and $\ket{\beta}$:
      \begin{align*}
        \ket{\psi'} = \begin{cases}
                        \ket{\alpha} & \text{with probability } \braket{\psi}{\alpha}\braket{\alpha}{\psi}\\
                        \ket{\beta}  & \text{with probability } \braket{\psi}{\beta}\braket{\beta}{\psi}
                      \end{cases}
      \end{align*}
      Measurement is refered to as a \textit{destructive operation} because it cannot 
      be reversed; once performed, we cannot recover the pre-measurement quantum state.
    
    \subsubsection{Quantum Gates}
      Quantum gates map from one quantum state to another. Gates are represented by a
      unitary matrix, $U$. (For a matrix $U$ to be unitary, 
      $UU^\dagger = U^\dagger U = I$.) Because gates are unitary, they are 
      \textit{reversible}, which means that applying gate $U$ to a qubit can be 
      undone by applying $U^{-1}$. 
      
      Also, gates may act on only a single qubit or 
      multiple. An example of a commonly used single qubit gate is the 
      \textit{Hadamard gate}:
      \begin{align*}
        H = \frac{1}{\sqrt{2}}
            \begin{pmatrix}
              1 & 1\\
              1 & -1\\
            \end{pmatrix}
      \end{align*}
      When applied to the computational basis states, the Hadamard gate maps
      $\ket{0} \rightarrow \ket{+}$ and $\ket{1} \rightarrow \ket{-}$. The
      Hadamard gate also has the useful property that $HH = I$; therefore, 
      $\ket{+} \rightarrow \ket{0}$ and $\ket{-} \rightarrow \ket{1}$.

      Other important single qubit gates are the Pauli operators: $X$, $Y$, and $Z$.
      Each of these rotate a qubit's state around the $x$-, $y$-, or $z$-axis when
      the qubit is represented in three-dimensional space. These gates are as follows:
      \begin{align*}
        X = \begin{pmatrix}
              0 & 1\\
              1 & 0
            \end{pmatrix}, 
        Y = \begin{pmatrix}
              0 & -i\\
              i & 0
            \end{pmatrix},
        Z = \begin{pmatrix}
              1 & 0\\
              0 & -1
            \end{pmatrix}
      \end{align*}

      Single qubit gates can be applied to a single qubit state of a multi-qubit
      system by using the tensor product. For example, to apply a Hadamard gate
      to the second qubit of $\ket{00}$:
      \begin{align*}
        (I \otimes H)\ket{00} = \ket{0+}
      \end{align*}
      Or to apply the Hadamrd gate to both qubits:
      \begin{align*}
        (H \otimes H)\ket{00} = \ket{++}
      \end{align*}

    An important multi-qubit gate is the \textit{controlled-U} gate (sometimes
    written $\wedge U$), where $U$ is a single qubit gate. In a controlled-U gate, 
    there's a ``control'' and ``target'' qubit. The operator $U$ is only applied to 
    the target qubit if the control qubit equals $\ket{1}$, and nothing is applied 
    otherwise. For example, consider the $X$ gate; when applied to a qubit the $X$ 
    gate swaps the amplitudes:
    \begin{align*}
      X \qstate{\alpha}{\beta} = \qstate{\beta}{\alpha}
    \end{align*}
    Now, consider the controlled-X gate, $\wedge X$, actings on the following states
    where the first qubit is the control and the second qubit the target:
    \begin{align*}
      \wedge X \ket{00} = \ket{00}\\
      \wedge X \ket{01} = \ket{01}\\
      \wedge X \ket{10} = \ket{11}\\
      \wedge X \ket{11} = \ket{10}
    \end{align*}
    In the cases where the first qubit was $\ket{1}$, the second qubit flipped its
    value and when the first qubit was $\ket{0}$, the state remained the same. 
    The controlled-X gate is typically referred to as the controlled-NOT gate 
    or \textit{CNOT}.

    The controlled-Z gate, sometimes referred too as the controlled-PHASE gate, will 
    have an important role in later sections of this paper.

    \subsubsection{Quantum Circuits}
      The quantum circuit model is a gate-based model of quantum computation,
      analgous to classical Boolean circuits. A quantum circuit first consists of
      a set of qubits prepared in some initial state. Then, quantum gates are
      sequentially applied to the qubits. Finally, the qubits are measured with
      respect to a basis. An example is depicted in Figure 1 (TODO).

  \subsection{Measurement-Based Quantum Computing}
    Measurement-Based Quantum Computing (MBQC) is another model
    of quantum computation different from the standard gate-based
    approach. One important model of MBQC is the \textit{cluster
    state model} [TODO; TODO]. The cluster state model typically involves 
    (1) the creation of a \textit{cluster state}, i.e., a 
    collection of entangled qubits, (2) the measurement of qubits 
    in different bases, and, in some variations, (3) the application of X and Z 
    \textit{corrections} using the Pauli operators. Importantly, 
    the basis of each measurement and whether corrections are 
    performed may be dependent on the outcome of earlier 
    measurements performed during the computation. The 
    computation is also performed in this order: entanglement, 
    measurement, correction.

    The cluster state of the computation is typically represented
    by performing a controlled-Z gate between qubits to entangle
    them. Computation then proceeds by measuring qubits one
    at a time, slowing disentangling the cluster. Because the
    entanglement of the cluster can only decrease as the
    computation progresses, the cluster state model is typically
    referred to as \textit{one-way quantum computation}.
    Various configurations of cluster states and their corresponding
    gate-based circuits are shown in Figure~\ref{fig:clusters}; these
    clusters can be composed together to form more complex computations.

    The cluster state model has had an important impact on 
    understanding the nature of entanglement in quantum
    computation and in helping build optical quantum computers 
    [TODO].

    \begin{figure}
      \begin{tikzpicture}  
        [scale=.9,auto=left,every node/.style={circle,fill=blue!20}]
          
        \node (a1) at (1,1) {$q_1$};  
        \node (a2) at (3,1) {$q_2$};  
        \node (a3) at (5,1) {$q_3$};
        
        \draw (a1) -- (a2); 
        \draw (a2) -- (a3);
    
      \end{tikzpicture}
      {
        % definitions for the circuit elements
    
        \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
        \def\gBxA{\op{R_x(-\beta)}\w\A{gBxA}}
    
        % definitions for bit labels and initial states
    
        \def\bA{\qv{q_{0}}{\psi}}
    
        % The quantum circuit as an xymatrix
    
        \xymatrix@R=5pt@C=10pt{
            \bA & \gAxA &\gBxA &\n
        %
        % Vertical lines and other post-xymatrix latex
        %
        }
      }
      \begin{flushleft}
        $\mathcal{J}(\alpha)(q_1, q_2); \mathcal{J}(\beta)(q_2,q_3)$
      \end{flushleft}
    \end{figure}
    
    \begin{figure}
      \begin{tikzpicture}  
        [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
          
        \node (a1) at (1,1) {$q_1$};  
        \node (a2) at (3,1) {$q_2$};  
        \node (a3) at (5,1) {$q_3$};
        \node (a4) at (7,1) {$q_4$};
        
        \draw (a1) -- (a2); 
        \draw (a2) -- (a3);
        \draw (a3) -- (a4);
    
      \end{tikzpicture}  
      {
        \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
        \def\gBxA{\op{R_x(-\beta)}\w\A{gBxA}}
        \def\gCxA{\op{R_z(-\gamma)}\w\A{gCxA}}
        \def\gDxA{\op{H}\w\A{gDxA}}
    
        % definitions for bit labels and initial states
    
        \def\bA{\qv{q_{0}}{\psi}}
    
        % The quantum circuit as an xymatrix
    
        \xymatrix@R=5pt@C=10pt{
            \bA & \gAxA &\gBxA &\gCxA &\gDxA &\n
        %
        % Vertical lines and other post-xymatrix latex
        %
        }
      }
      \begin{flushleft}
        $\mathcal{J}(\alpha)(q_1, q_2); \mathcal{J}(\beta)(q_2,q_3); \mathcal{J}(\gamma)(q_3,q_4)$
      \end{flushleft}
    \end{figure}
    
    \begin{figure}
      \begin{tikzpicture}  
        [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
          
        \node (a1) at (1,3) {$q_1$};
        \node (a2) at (1,1) {$q_2$};  
    
        \node (a3) at (3,3) {$q_3$};
        \node (a4) at (3,1) {$q_4$};  
        
        \draw (a1) -- (a2); 
        \draw (a1) -- (a3);
        \draw (a2) -- (a4);
    
      \end{tikzpicture}  
      {
        \def\gAxA{\b\w\A{gAxA}}
        \def\gAxB{\b\w\A{gAxB}}
        \def\gBxA{\op{R_z(-\alpha)}\w\A{gBxA}}
        \def\gBxB{\op{R_z(-\beta)}\w\A{gBxB}}
        \def\gCxA{\op{H}\w\A{gCxA}}
        \def\gCxB{\op{H}\w\A{gCxB}}
        
        % definitions for bit labels and initial states
        
        \def\bA{\qv{q_{0}}{\psi}}
        \def\bB{\qv{q_{1}}{\varphi}}
        
        % The quantum circuit as an xymatrix
        
        \xymatrix@R=5pt@C=10pt{
            \bA & \gAxA &\gBxA &\gCxA &\n
        \\  \bB & \gAxB &\gBxB &\gCxB &\n
        %
        % Vertical lines and other post-xymatrix latex
        %
        \ar@{-}"gAxA";"gAxB"
        }
      }
      \begin{flushleft}
        $\wedge\mathcal{Z}(q_1,q_2); \mathcal{J}(\alpha)(q_1, q_3); \mathcal{J}(\beta)(q_2,q_4)$
      \end{flushleft}
    
      \begin{tikzpicture}  
        [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
          
        \node (a1) at (1,3) {$q_1$};
        \node (a2) at (1,1) {$q_2$};  
    
        \node (a3) at (3,3) {$q_3$};
        \node (a4) at (3,1) {$q_4$};  
        
        \draw (a3) -- (a4); 
        \draw (a1) -- (a3);
        \draw (a2) -- (a4);
    
      \end{tikzpicture}  
      {
        \def\gAxA{\op{R_z(-\alpha)}\w\A{gAxA}}
        \def\gAxB{\op{R_z(-\beta)}\w\A{gAxB}}
        \def\gBxA{\op{H}\w\A{gBxA}}
        \def\gBxB{\op{H}\w\A{gBxB}}
        \def\gCxA{\b\w\A{gCxA}}
        \def\gCxB{\b\w\A{gCxB}}
        
        % definitions for bit labels and initial states
        
        \def\bA{\qv{q_{0}}{\psi}}
        \def\bB{\qv{q_{1}}{\varphi}}
        
        % The quantum circuit as an xymatrix
        
        \xymatrix@R=5pt@C=10pt{
            \bA & \gAxA &\gBxA &\gCxA &\n
        \\  \bB & \gAxB &\gBxB &\gCxB &\n
        %
        % Vertical lines and other post-xymatrix latex
        %
        \ar@{-}"gCxA";"gCxB"
        }
      }
      \begin{flushleft}
        $\mathcal{J}(\alpha)(q_1, q_3); \mathcal{J}(\beta)(q_2,q_4); \wedge\mathcal{Z}(q_1,q_2)$
      \end{flushleft}
    \end{figure}
    
    \begin{figure}
      \begin{tikzpicture}  
        [scale=.9,auto=center,every node/.style={circle,fill=blue!20}]
          
        \node (a1) at (1,3) {$q_1$};
        \node (a2) at (1,1) {$q_2$};  
    
        \node (a3) at (3,3) {$q_3$};
        \node (a4) at (3,1) {$q_4$};  
        
        \draw (a1) -- (a2);
        \draw (a3) -- (a4); 
        \draw (a1) -- (a3);
        \draw (a2) -- (a4);
    
      \end{tikzpicture}  
      {
        \def\gAxA{\b\w\A{gAxA}}
        \def\gAxB{\b\w\A{gAxB}}
        \def\gBxA{\op{R_z(-\alpha)}\w\A{gBxA}}
        \def\gBxB{\op{R_z(-\beta)}\w\A{gBxB}}
        \def\gCxA{\op{H}\w\A{gCxA}}
        \def\gCxB{\op{H}\w\A{gCxB}}
        \def\gDxA{\b\w\A{gDxA}}
        \def\gDxB{\b\w\A{gDxB}}
        
        % definitions for bit labels and initial states
        
        \def\bA{\qv{q_{0}}{\psi}}
        \def\bB{\qv{q_{1}}{\varphi}}
        
        % The quantum circuit as an xymatrix
        
        \xymatrix@R=5pt@C=10pt{
            \bA & \gAxA &\gBxA &\gCxA &\gDxA &\n
        \\  \bB & \gAxB &\gBxB &\gCxB &\gDxB &\n
        %
        % Vertical lines and other post-xymatrix latex
        %
        \ar@{-}"gAxA";"gAxB"
        \ar@{-}"gDxA";"gDxB"
        }
      }
      \begin{flushleft}
        $\wedge\mathcal{Z}(q_1,q_2); \mathcal{J}(\alpha)(q_1, q_3); \mathcal{J}(\beta)(q_2,q_4); \wedge\mathcal{Z}(q_1,q_2)$
      \end{flushleft}
    
      \caption{Cluster Conversion}
      \label{fig:clusters}
    \end{figure}
    
  \subsection{The Measurement Caclulus}
    The \textit{measurement calculus} is a variation of the cluster
    state model formalized by Danos et al []. It provides a clear
    syntax and semantics to the cluster state operations along
    with rewriting rules for simpliying sequences of commands.
    The measurement calculus, like the cluster state model in general,
    is universal; therefore, it can compute anything that
    the standard gate-based model can.

    \subsubsection{Commands}
      The measurement calculus consists of four commands: 
      preparation ($N$),
      entanglement ($E$), measurement ($M$), and then Pauli
      corrections ($X$ and $Z$).

      The preparation command, $N_i$, initializes qubit $i$
      to the $\ket{+}$ state.
      
      The entanglement command, $E_{ij}$, entangles qubits
      $i$ and $j$ by performing a controlled-Z gate between
      them with $i$ the control and $j$ the target.

      The measurement command, $M_i^\alpha$, measures
      qubit $i$ with the following basis states:
      \begin{align*}
        \ket{+_\alpha} &= \frac{1}{\sqrt{2}}(\ket{0} + e^{i\alpha}\ket{1})\\
        \ket{-_\alpha} &= \frac{1}{\sqrt{2}}(\ket{0} - e^{i\alpha}\ket{1})
      \end{align*}
      where $\alpha \in [0, 2\pi]$; $\alpha$ is referred to as
      \textit{the angle of measurement}. Notice the when $\alpha = 0$,
      measurement is performed with the $\ket{+}$ and $\ket{-}$ basis
      states.

      The correction commands, $X_i$ and $Z_i$ apply the Pauli
      $X$ or $Z$ gates, respectively, to qubit $i$.

      The measurement and correction commands may be dependent
      on the results of past measurements performed. The outcome
      of a measurement on qubit $i$ is denoted as $s_i$ where
      \begin{align*}
        s_i = \begin{cases}
                0 &\text{if the qubit collapsed to } \ket{+_\alpha}\\
                1 &\text{if the qubit collapsed to } \ket{-_\alpha}
              \end{cases}
      \end{align*}
      Dependent commands use \textit{signals} to determine the 
      operation performed. Signals are the summation of the outcome 
      of certain qubits, performed in $\mathbb{Z}_2$. In other words,
      signal $s = \left(\sum_{i \in Q}{s_i}\right) \text{ mod } 2$ where $Q$ is the set of qubits
      the commands depends on. $Q$ is referred to as the \textit{domain} 
      of a signal. Therefore, calculating the signal is a function
      which maps subsets of qubits to either $0$ or $1$: 
      $f: \wp(Q_{All}) \rightarrow \{0, 1\}$.
      
      Dependent corrections are written $X^s_i$ and $Z^s_i$.
      The operation is performed if $s = 1$ and not performed if
      $s = 0$. For example, in the case of $X^s_i$, $X^1_i = X_i$
      and $X^0_i = I_i$ where $I$ is simply the identify matrix.
      
      Dependent corrections are written as 
      \begin{align*}
        {}^t[M_i^\alpha]^s = M_i^{(-1)^s\alpha + t\pi}
      \end{align*}
      where $t$ and $s$ are signals.

    \subsubsection{Patterns}
      Essentially, patterns consist of a finite sequence of 
      commands and three sets of qubits: $V$, $I$, and $O$.
      $V$ is the computational space, i.e., the set of all qubits
      used in the computation. $I$ is the set of input qubits
      and $O$ is the set of output qubits. Moreover, in this
      paper, a sequence of commands, $A_1 \dots A_n$ is read from
      left to right. [TODO: footnote noting original paper
      read sequences from right to left.] Note that
      $I \cup O \subseteq V$ and the sets $I$ and $O$
      may share the same qubits -- i.e., $I \cap O$ does not
      necessarily equal $\varnothing$.

      Patterns must abide by the following constraints:
      \begin{enumerate}
        \item no command depends on an outcome not yet measured
        \item no command acts on a qubit already measured
        \item no command acts on a qubit not yet prepared, unless it is an input qubit
        \item a qubit $i$ is measured if and only if $i$ is not an output
      \end{enumerate}
      The constraints ensure that a pattern is well-formed so
      that execution of the commands makes sense. 

      Moreover, the following set of patters is universal:
      \begin{align*}
        \wedge \mathcal{Z}(i, j) &:= E_{ij}\\
        \mathcal{J}(\alpha)(i, j) &:= E_{ij}; M^{-\alpha}_i; X^{s_i}_j
      \end{align*}
      where $V = \{i, j\}$ for both patterns; for $\wedge\mathcal{Z}$, 
      $I = O = \{i,j\}$; for $\mathcal{J}(\alpha)(i, j)$, $I = \{i\}$ and
      $O = \{j\}$. Equivalently, $\mathcal{J}(\alpha) = R_z(\alpha); H$;
      therefore, $\mathcal{J}(0) = H$.
      Examples providing further clarification is provided in section
      3.

    \subsubsection{Standardization}
      Standarizing a pattern takes an arbitrary, but stil well-formed,
      sequence of commands and rewrites the pattern to put commands in
      the following order: preparations, entanglement, measurement, corrections.
      The pattern is rewritten using a set of rewriting rules laid
      out in [TODO]. Once standardized, the pattern is simplified and in 
      the proper format resembling cluster state computation.
      
      Importantly, the rewriting rules perserve the semantics of the
      pattern; therefore, the standardized pattern will result
      in the same computation as the original, non-standardized one.

      The rewriting rules are as follows:
      \begin{align*}
        X^s_i; E_{ij} &\Rightarrow E_{ij}; Z^s_j; X^s_i\\
        X^s_j; E_{ij} &\Rightarrow E_{ij}; Z^s_i; X^s_j\\
        Z^s_i; E_{ij} &\Rightarrow E_{ij}; Z^s_i\\
        Z^s_j; E_{ij} &\Rightarrow E_{ij}; Z^s_j\\
        X^r_i; {}^t[M^\alpha_i]^s &\Rightarrow {}^t[M^\alpha_i]^{s+r}\\
        Z^r_i; {}^t[M^\alpha_i]^s &\Rightarrow {}^{r+t}[M^\alpha_i]^s
      \end{align*}
      and the \textit{free commutation rules},
      \begin{align*}
        A_{\vec{k}}; E_{ij} &\Rightarrow E_{ij}; A_{\vec{k}} &\text{where $A$ is not an enntanglement}\\
        X^s_i; A_{\vec{k}} &\Rightarrow A_{\vec{k}}; X^s_i &\text{where $A$ is not a correction}\\
        Z^s_i; A_{\vec{k}} &\Rightarrow A_{\vec{k}}; Z^s_i &\text{where $A$ is not a correction}\\
      \end{align*}
      where $\vec{k}$ is a set of qubits the command is acting on.

      An example of applying these rules is shown in the following section.

  \subsection{Existing Quantum Programming Languages}
  
    The extensive work done both in academia and industry to build quantum systems, 
    manufacture relevant quantum algorithms, and explain existing research has led to
    an influx of quantum programming languages and frameworks with unique features
    that suit different needs. In this section, we will provide a general overview of the
    quantum programming languages in hopes to highlight the distinctions of this measurement
    based quantum programming language [TODO - insert mclang name here]. While the sample size of 
    quantum programming languages and frameworks is large, for the scope of this paper, 
    we will be focusing on languages that are directly used in our work.

    \textbf{TODO: make this cleaner, add Silq}
    The quantum programming languages we will be covering can be separated into three
    different categories: \textit{feature-rich}, \textit{intermediate representations}, 
    and \textit{TODO: should we talk about Q sharp/quipper and languages that aren't relevant?}

    \subsubsection{Cirq}
      Cirq is a popular gate-based quantum programming framework focused on running 
      programs on noisy intermediate-scale quantum computers[TODO: cite], 
      providing the users  with functionality to interact and develop programs 
      with hardware in mind. In Cirq, users are able to develop circuits with 
      or without hardware topology constraints, generate fake noise models 
      when running circuits in simulation, and assess error rates on real 
      devices via the Google Quantum Computing Service[TODO: cite].

      Written as a library on top of Python, Cirq offers both an extensive
      amount of control over the low-level components of quantum programming
      while also providing abstractions for users to explore and develop 
      quantum algorithms hassle-free. It also offers user-friendly features like
      the Cirq-web package[TODO: cite], which allow for 3D interactive
      visualizations of quantum states and circuits enabling researchers and 
      educators to easily understand what they are creating. Cirq also takes
      advantage of Python's broad feature set to make building and testing 
      complex circuits as intuitive and accessible as possible for programmers
      new to the framework, while also leveraging these same features in their
      own library so the learning curve for the language is as small as possible.

      While Cirq is a strong tool for gate-based quantum programming, it does
      not directly support programs with operations depending on measurement 
      results, a key limitation when attempting to run measurement-based quantum
      programs. One workaround for this would be to gather the quantum state at
      the end of a circuit simulation, decide the next state based off of the
      measurement result of that state, and start a new simulation starting in the
      previous state. This workaround is not all-encompassing, however, since this
      method is only possible in simulation. \textbf{TODO: Ask question about 
      non-deterministic circuits in general on NISQ devices? Are they even possible?}

    \subsubsection{OpenQASM}
      OpenQASM (Open Quantum Assembly Language) is a gate-based intermediate
      representation of quantum programs which can be directly read by quantum
      processors. \cite{cross2017open} It is a widely
      adopted intermediate representation, supported by many quantum 
      programming framework, including Qiskit, Cirq, and Pennylane.

      Most quantum programmers do not build programs using OpenQASM, similarly to
      how most classical programmers do not build programs using x86 or ARM. Instead,
      OpenQASM output is generated by higher level quantum programs and serves as a
      standard for representation and execution of quantum circuits. Most Python quantum
      programming frameworks include functionality to build circuits from OpenQASM and 
      vice versa. This versatility allows users to take advantage of features offered
      by one organization that may not be offered by another. For example, since 
      Google's Quantum Computing Service is not yet available to the public, a circuit
      written in Cirq can be converted to OpenQASM, imported into the IBM Quantum
      Experience platform which provides cloud access to quantum systems to the public, 
      and run on a real device.

    \subsubsection{PyZX}
      PyZX is a Python library implementing the ZX-calculus\cite{vandewetering2020zxcalculus}, allowing the creation,
      visualization, and automated rewriting of large-scale quantum circuits. \cite{kissinger2020Pyzx}. It supports conversion of ZX-calculus
      diagrams to generic circuit models, and to QASM. 

      PyZX does not offer simulation of quantum circuits, but allows circuits to be 
      represented in terms of ZX-calculus, rewritten and potentially optimized accordingly, 
      and then represented in QASM, QC[TODO: cite], or Quipper[TODO: cite] for use with
      other languages. 

      The origins of the ZX calculus have ties to measurement-based quantum 
      computation. Since graph states
      have simple representations in ZX-diagrams, measurement-based computation models
      can be easily represented in the ZX-calculus. 

    \subsubsection{Silq}
      Silq is a unique quantum programming language that automatically uncomputes
      temporary values in quantum programs, making quantum programs shorter and much more
      readable. [TODO: cite - https://files.sri.inf.ethz.ch/website/papers/pldi20-silq.pdf] 
      It also abstracts away details of quantum programs that are necessary to 
      include in programming languages like Cirq, allowing developers to focus solely on
      building programs that leverage the power of quantum computation without worrying
      about concepts present in the circuit model.
    
      \textbf{In the background section, should we talk about why we picked 
      each language?}


